Weak Convergence (IIA) - Functional and Random Aspects of the Univariate Extreme Value Theory

The univariate extreme value theory deals with the convergence in type of powers of elements of sequences of cumulative distribution functions on the real line when the power index gets infinite. In terms of convergence of random variables, this amounts to the the weak convergence, in the sense of probability measures weak convergence, of the partial maximas of a sequence of independent and identically distributed random variables. In this monograph, this theory is comprehensively studied in the broad frame of weak convergence of random vectors as exposed in Lo et al.(2016). It has two main parts. The first is devoted to its nice mathematical foundation. Most of the materials of this part is taken from the most essential Lo\`eve(1936,177) and Haan (1970), based on the stunning theory of regular, pi or gamma variation. To prepare the statistical applications, a number contributions I made in my PhD and my Doctorate of Sciences are added in the last chapter of the last chapter of that part. Our real concern is to put these materials together with others, among them those of the authors from his PhD dissertations and Science doctorate thesis, in a way to have an almost full coverage of the theory on the real line that may serve as a master course of one semester in our universities. As well, it will help the second part of the monograph. This second part will deal with statistical estimations problems related to extreme values. It addresses various estimation questions and should be considered as the beginning of a survey study to be updated progressively. Research questions are tackled therein. Many results of the author, either unpublished or not sufficiently known, are stated and/or updated therein.

==> evt_math_spr_en.tex <==
\chapter{Special Properties and Refinements} \label{evtspr}

We begin with Von Mises types conditions. If a distribution function $F$ has first or second derivative function, we have specific conditions ensurung that $F$ is in the extreme value domain of attraction. These conditions have been showed as necessary under some monotonicity assumptions by \cite{dehaan}. The first part of this
is a restitution of the works of de Haan in the cited monograph. \\

\noindent \textbf{II - Von Mises and de Haan conditions based on derivatives}.\\

\subsection{Von Mises condition for the Frechet's domain}. $ $\\

\noindent We have the following result.\\

\begin{proposition} \label{evtspr.prop.01} Let $F$ be \textit{cdf} on $\mathbb{R}$ such that $uep(F)=+\infty$ and there exists $x_0>0$ such that the derivative function $F^{\prime}(x)$ exists for $x \geq x_0$. Let $\alpha$ be positive real number. The following assertions hold.\\

\noindent (a) $F \in D(H_{1/\alpha})$ whenever holds
 

\begin{equation}
\lim_{x\rightarrow +\infty} \frac{xF^{\prime}(x)}{1-F(x)}=\alpha. \label{evtspr.01}.
\end{equation}

\noindent (b) If $F^{\prime}(x)$ is non-increasing on $[x_0, +\infty[$ and $F \in D(H_{1/\alpha})$, then Formula (\ref{evtspr.01}) holds.
\end{proposition}

\bigskip \noindent \textbf{Proof of Proposition \ref{evtspr.prop.01}}.\\

\noindent \textbf{Proof of Point (a)}. Let us suppose that there exists $upe(F)=+\infty$ such that the derivative function $F^{\prime}(x)$ exists for $x \geq x_0$ and that Formula \ref{evtspr.01} holds. Then $F^{\prime}$ is non-negative and measurable on $[x_0, \ +\infty[$. Thus for $x\geq x_0$,

\begin{equation}
1-F(x)=\int_{x}^{+\infty} F^{\prime}(t) dt. \label{evtspr.02}
\end{equation}

\noindent Hence Formula \ref{evtspr.01} becomes, as $x\rightarrow +\infty$,

$$
\frac{xF^{\prime}(x)}{1-F(x)}=\frac{xF^{\prime}(x)}{\int_{x}^{+\infty} F^{\prime}(t) dt} \rightarrow \alpha. 
$$

\noindent  By Lemma \ref{evt.karamata.lem3} in Chapter \ref{evt}, $F^{\prime} \in RV(-\alpha-1, +\infty)$, and then $1-F(x) \sim \alpha xF^{\prime}(x)$ is in
$RV(-\alpha, +\infty)$, which by Theorem \ref{evt.extdom.charac.frechet}, belongs to $D(H_{1/\alpha}$.\\



\noindent \textbf{Proof of Point (b)}. Let us suppose that there exists $upe(F)=+\infty$ such that the derivative function $F^{\prime}(x)$ exists for $\leq \geq x_0$ and is non-increasing. Let us prove that Formula \ref{evtspr.01} holds. Formula (\ref{evtspr.02}) is still valid. By using the right change of variable and straightforward computations, we get for $1\leq x,y$ and $t\geq x_0$,

\begin{eqnarray}
A(x,y,t)&=&\left(\frac{1-F(tx)}{1-F(t)}\right)-\left(\frac{1-F(tx)}{1-F(t)}\right) \label{evtspr.02b}\\
&=&\frac{1}{1-F(t)}\int_{tx}^{ty} F^{\prime}(s)ds \notag \\
&=&\frac{1}{1-F(t)}\int_{x}^{y} tF^{\prime}(ts)ds \notag\\
&=& \frac{tF^{\prime}(t)}{1-F(t)}\int_{x}^{y} \frac{F^{\prime}(ts)}{F^{\prime}(t)}ds \notag\\
\end{eqnarray}

\noindent Hence for $1<x<y$ and $t\geq x_0$, we get by the monotonicity of $F^{\prime}$ (which ensures that $F^{\prime}(ts)\leq F^{\prime}(t)$ since $ts>t$ with 
$x>1$ and $t\geq 0$), that 

$$
A(x,y,t)\leq (y-x) \frac{tF^{\prime}(t)}{1-F(t)}.
$$

\noindent By Theorem \ref{evt.extdom.charac.frechet} and Formula Formula \ref{evtspr.01}, we get, as $t\rightarrow +\infty$

$$
x^{-\alpha}-y^{-\alpha} \leq (y-x) \liminf_{t\rightarrow +\infty} \frac{tF^{\prime}(t)}{1-F(t)},
$$

\noindent which is

$$
\liminf_{t\rightarrow +\infty} \frac{tF^{\prime}(t)}{1-F(t)} \leq -\frac{y^{-\alpha}-x^{-\alpha}}{y-x},
$$

\noindent For all $1<x<y$. By doing $y\downarrow x$, we get the derivative of the function $x^{-\alpha}$ in the latter formula, which leads to

$$
\liminf_{t\rightarrow +\infty} \frac{tF^{\prime}(t)}{1-F(t)} \leq \alpha x^{-(\alpha+1)}
$$

\noindent For all $x>1$. We get, by letting $x\downarrow 1$in the formula above, that


\begin{equation}
\liminf_{t\rightarrow +\infty} \frac{tF^{\prime}(t)}{1-F(t)} \leq \alpha. \label{evtspr.02a}
\end{equation}

\noindent Similarly, we have for $1/2 <x<y<1$ and $t\geq x_0$, we 

\begin{eqnarray}
A(x,y,t)&=& \frac{tF^{\prime}(t)}{1-F(t)}\int_{x}^{y} \frac{F^{\prime}(ts)}{F^{\prime}(t)}ds \notag\\
&\geq & (y-x) \frac{tF^{\prime}(t)}{1-F(t)}.
\end{eqnarray}

\noindent From there, by still using similar methods that

\begin{equation}
\limsup_{t\rightarrow +\infty} \frac{tF^{\prime}(t)}{1-F(t)} \leq \alpha. \label{evtspr.02c}.
\end{equation}

\noindent The combination between Formulas (\ref{evtspr.02c}) and (\ref{evtspr.02c}) puts an end to the proof.$\blacksquare$\\


\subsection{Von Mises condition for the Weibull's domain}. $ $\\

\noindent We only need to use the correspondence between Frechet's and Weibull's domain as in Theorem \ref{evt.extdom.charac.weibull} in Chapter \ref{evt}, whihx is the following : $F\in D(H_{-1/\alpha})$ with $\alpha>0$ if and only if $uep(F)<+\infty$ and the \textit{cdf} $F(uep(F)-1/.) \in D(H_{\alpha})$.\\

\noindent This remark leads to the following result.
 

\begin{proposition} \label{evtspr.prop.02} Let $F$ be \textit{cdf} on $\mathbb{R}$ such that $uep(F)<+\infty$ and there exists $x_0>0$ such that the derivative function $F^{\prime}(x)$ exists for $x_0\leq x \leq uep(F)$. Let $\alpha$ be positive real number. The following assertions hold.\\

\noindent (a) $F \in D(H_{-1/\alpha})$ whenever holds
 

\begin{equation}
\lim_{x\rightarrow uep(F)^{-}} \frac{(uep(F)-x) F^{\prime}(x)}{1-F(x)}=\alpha. \label{evtspr.03}.
\end{equation}

\noindent (b) If $F^{\prime}(x)$ is non-increasing on $[x_0, uep(F)[$ and $F \in D(H_{-1/\alpha})$, then Formula (\ref{evtspr.03}) holds.
\end{proposition}


\subsection{Von Mises condition for the Gumbel's domain}. $ $\\

\noindent Here, we have two results, the first, which is a preparation of the second, us the following.\\
 

\begin{proposition} \label{evtspr.prop.03} Let $F$ be \textit{cdf} on $\mathbb{R}$ and there exists $x_0>0$ such that the derivative function $F^{\prime}(x)$ exists for $x_0\leq x < uep(F)$. Define

$$
\ell(F,x)=:\ell(x)=\frac{F^{\prime}(x) \int_{x}^{uep(F)} 1-F(t) \ dt}{1-F(x)}, \ u<upe(F).
$$

\noindent The following assertions hold.\\

\noindent (a) $F \in D(H_{0})$ whenever holds $\ell(x)\rightarrow 1$ as $t\rightarrow uep(F)^{-}$.\\
 

\noindent (b) If $F^{\prime}(x)$ is non-increasing on $[x_0, uep(F)[$ and $F \in D(H_{0})$, then $\ell(x)\rightarrow 1$ as $t\rightarrow uep(F)^{-}$.
\end{proposition}


\bigskip \noindent The second and final one is certainly the most important.


\begin{proposition} \label{evtspr.prop.04} Let $F$ be \textit{cdf} on $\mathbb{R}$ and there exists $x_0>0$ such that the second derivative function $F^{\prime\prime}(x)$ exists for $x_0\leq x < uep(F)$. Suppose that : (H) there exists $x_0<uep(F)$ such that $1-F^{\prime}(x)>0$ for $x_0\leq x<uep(F)$ and $F^{\prime}(x)\downarrow 0$ as $x \uparrow uep(F)$. Let us define for $x_0\leq x <uep(F))$,

$$
q(F,x)=\frac{F^{\prime\prime}(x)(1-F(x))}{F^{\prime}(x)^2}.
$$

\noindent The following assertions hold.\\


\noindent (a) $F \in D(H_{0})$ whenever holds
 

\begin{equation}
\lim_{x\rightarrow uep(F)^{-}} q(F,x)=-1. \label{evtspr.04}.
\end{equation}

\noindent (b) If $F^{\prime\prime}(x)$ is non-decreasing on $[x_0, uep(F)[$ and $F \in D(H_{0})$, then Formula (\ref{evtspr.04}) holds.
\end{proposition}


\bigskip \noindent \textbf{Proof of Proposition \ref{evtspr.prop.03}}.\\

\noindent \textit{Proof of Point (a)}. If $\ell(x)\rightarrow 1$ as $x\rightarrow uep(F)^{-}$, then there exists $x_0<uep(F)$ that 
$k(x)=\int_{x}^{uep(F)} 1-F(t) \ dt$ is finite for $x_0\leq x <uep(F)$. It follows that the asymptotic moment function 
$r(x)=R(F,x)=k(x)/(1-F(x))$ is finite $x_0\leq x<uep(F)$ We have 

$$
-\frac{1}{r(x)}=\frac{dk(x)}{k(x)}, \ x_0\leq x <uep(F).
$$

\noindent By integrating on $[x_0, x]$ for $x_0\leq x<uep(F)$, and by reminding the definition of $k(.)$, 

\begin{equation} \label{evtspr.04a}
(1-F(x))/r(x)= k(x_0) \exp \left( \int_{x_0}^{x}-\frac{1}{r(t)} dt \right), \ x_0\leq x<uep(F).
\end{equation}

\noindent We may also see, by an easy computation that $r^{\prime}(x)=-1+\ell(x) \rightarrow 0$ as $x\rightarrow uep(F)^{-}$. Finally, we have for $x_0\leq x<uep(F)$,

$$
\int_{x_0}^{x} \frac{-1+\ell(t)}{r(t)}dt=\int_{x_0}^{x} \frac{dr(t)}{r(t)}=\log r(x) -\log r(x_1),
$$

\noindent which leads to

\begin{equation} \label{evtspr.04b}
r(x)= r(x_0) \exp \left( \int_{x_0}^{x} \frac{-1+\ell(t)}{r(t)} dt \right),
\end{equation}

\noindent for $x_0\leq x<uep(F)$. By combining Formulas (\ref{evtspr.04a}) and (\ref{evtspr.04b}), we obtain for $x_0\leq x<uep(F)$,

\begin{equation} \label{evtspr.04c}
1-F(x)= k(x_0)r(x_0) \exp \left( \int_{x_0}^{x} \frac{\ell(x)}{r(t)} dt \right), \ x_0\leq x<uep(F).
\end{equation} 

\noindent In view of Theorem (\ref{evtp.theo.08}) in Chapter \ref{evtp}, we may conclude that $F \in D(H_0)$ if we check that $r(x) \rightarrow 0$ as $x\rightarrow uep(F)^{-}$ for $uep(F)^{-}$ finite. But this follows from $g(x)=r(x)/r^{^\prime}(x)$,  $x_0\leq x<uep(F)$ and $r^{\prime}(x)=-1+\ell(x) \rightarrow 0$ as $x\rightarrow uep(F)^{-}$, whatever be $uep(F)$.$\square$\\

\bigskip \noindent \textbf{Proof of Point (b)}. Suppose that $F^{\prime}$ is non-increasing on $[x_0,uep(F)[$ and that $F \in D(H_0)$. Set $r(x)=R(F,x)$. By , we have for all couples of real numbers $x$ and $y$, as $t\rightarrow uep(F)^{-}$,

\begin{equation} \label{evtspr.05a}
\Gamma(F,x,r(t),t)-\Gamma(F,y,r(t),t) \rightarrow e^{-x}-e^{-y}.
\end{equation}

\noindent Since

$$
\Gamma(F,x,r(t),t)-\Gamma(F,y,r(t),t)=\frac{1}{1-F(t)} \int_{xr(t)+t}^{yr(t)+t} F^{\prime}(s)ds
$$

\noindent we have , by the change of variables $s=ur(t)+t$,

\begin{eqnarray}
&&\Gamma(F,x,r(t),t)-\Gamma(F,y,r(t),t) \label{evtspr.05b}\\
&=&\frac{1}{1-F(t)} \int_{x}^{y} F^{\prime}(ur(t)+t)r(t)du \\
&=&\frac{r(t)F^{\prime}(t)}{1-F(t)} \int_{x}^{y} \frac{F^{\prime}(ur(t)+t))}{F^{\prime}(t)}du \notag\\
&=& g(t) \int_{x}^{y} \frac{F^{\prime}(ur(t)+t))}{F^{\prime}(t)}du 
\end{eqnarray}

\noindent Let us fix $0<x\leq u <y$. By Lemma \ref{evtp.lem.01} in Chapter \ref{evtp}, there exists $x_1$, $x_0\leq x_1<uep(F)$ such that we have 
$ur(t)+t <uep(F)$ uniformly in $u \in [x, \ y]$ for $x_1\leq t <uep(F)$. Combined with the non-increasingness of $F^{\prime}$ on $[x_1,uep(F)[$ and knowing that
$r(t)>0$ for $x_1\leq t <uep(F)$, we get that
$$
\frac{F^{\prime}(ur(t)+t))}{F^{\prime}(t)} \leq 1,
$$

\noindent uniformly in $u \in [x, \ y]$ for $x_1\leq t <uep(F)$. All this, combined with Formula \ref{evtspr.05a} and Formula \ref{evtspr.05b}, gives as $t\rightarrow uep(F)^{-}$,
 

\begin{equation} \label{evtspr.05c}
 \rightarrow e^{-x}-e^{-y} \leq (\liminf_{t\rightarrow uep(F)^{-}} g(t))(y-x).
\end{equation}

\noindent By applying the same reasoning for $x\leq y<0$, we would get

\begin{equation} \label{evtspr.05d}
 \rightarrow e^{-x}-e^{-y} \geq (\limsup_{t\rightarrow uep(F)^{-}} g(t))(y-x).
\end{equation}

\noindent By letting $y\downarrow x$ in (\ref{evtspr.05c}) and (\ref{evtspr.05d}), by using the definition of the derivative of the function $e^{-x}$ and by 
letting $x\downarrow 0$ in (\ref{evtspr.05c}) and $x\uparrow 0$ (\ref{evtspr.05d}), we get that

$$
\lim_{t\rightarrow uep(F)^{-}} g(t),
$$

\noindent which was the target.\\


\bigskip \noindent \textbf{Proof of Proposition \ref{evtspr.prop.04}}.\\

\noindent \textbf{Proof of Point (a)}. Let Formula (\ref{evtspr.04}) holds. Then, necessarily, there exists $x_0<uep(F)$ such that $F^{\prime\prime}(x)$ is finite and negative for $x_0\leq x <uep(F)$. Then $F^{\prime}$ is strictly non-decreasing and continuous on $]x_0,uep(F)[$. \\

\noindent Because of hypothesis (H), then the function $G$ on $\mathbb{R}$ defined by
$$
G(x)= (1-F^{\prime}(x)) 1_{(x_0 \leq x <uep(F))}, \ x<uep(F)
$$ 

\noindent is \textit{cdf} on $\mathbb{R}$ with $upe(G)=uep(F)$. But this implies that

\begin{equation} \label{evtspr.06a}
1-F(x)= 1 - \int_{x}^{uep(G)} 1-G(t) \ dt, \ \ x_0\leq x<uep(F)
\end{equation}

\noindent and, by using the notation Proposition \ref{evtspr.prop.03}, we hage

$$
\ell(G,x)=-q(F,x), \ x_0 \leq x <uep(F).\\
$$ 

\noindent Hence, Formula (\ref{evtspr.04}) implies that $\ell(G,x)\rightarrow 1$ as $x \uparrow uep(G)$, which implies through Proposition \ref{evtspr.prop.03} that $G \in D(H_0)$. Next, by taking Formula (\ref{evtspr.06a}) into account and by applying Proposition \ref{evtp.prop.04A}, we get that $F \in D(H_0)$.\\


\noindent \textbf{Proof of Point (b)}. Still because of Hypothesis (H), the function $G$ defined on $\mathbb{R}$ by
$$
G(x)= (1-F^{\prime}(x)) 1_{(x_0 \leq x <uep(F))}, \ x<uep(F)
$$ 

\noindent is \textit{cdf} on $\mathbb{R}$ with $upe(G)=uep(F)$. And, by Formula (\ref{evtspr.06a}) and by using the notation in Formulas (\ref{evtp.quot21b}) and  (\ref{evtp.quot21b}), we have
$$
\ell(F,x)=H(G,x), \ x_0\leq x <upe(F),
$$

\noindent and we should have in mind that $uep(G)=uep(F)$. Now, since $F^{\prime}$ is non-increasing and $F\in D(H_0)$, Proposition \ref{evtspr.prop.03} implies $\ell(x,F)$, and then $H(G,x)$, tends to the unity as $x \uparrow uep(F)$. Hence, by Theorem \ref{evtp.theo.08} in Chapter \ref{evtp}, we get $G\in D(H_0)$. Now, for values near $uep(G)$, we have $G^{\prime}(x)=-F^{\prime\prime}(x)$0=. Thus, then $G^{\prime}$ is non-increasing for values near $uep(G)$. Hence, \ref{evtspr.prop.03} implies $q(x,F)=-\ell(x,G)$ converges to $-1$ as $x \rightarrow uep(F)^{-1}$.$\blacksquare$\\
\endinput
